Performance Modeling and Prediction for Dense Linear Algebra

This dissertation introduces measurement-based performance modeling and prediction techniques for dense linear algebra algorithms. As a core principle, these techniques avoid executions of such algorithms entirely, and instead predict their performance through runtime estimates for the underlying compute kernels. For a variety of operations, these predictions allow to quickly select the fastest algorithm configurations from available alternatives. We consider two scenarios that cover a wide range of computations: To predict the performance of blocked algorithms, we design algorithm-independent performance models for kernel operations that are generated automatically once per platform. For various matrix operations, instantaneous predictions based on such models both accurately identify the fastest algorithm, and select a near-optimal block size. For performance predictions of BLAS-based tensor contractions, we propose cache-aware micro-benchmarks that take advantage of the highly regular structure inherent to contraction algorithms. At merely a fraction of a contraction's runtime, predictions based on such micro-benchmarks identify the fastest combination of tensor traversal and compute kernel.

==> Makefile <==
PDFLATEX = pdflatex -shell-escape

TARGET = main.pdf

default: figs once

# internals below

TARGETSTEM = $(TARGET:.pdf=)

once: preamble.fmt
	$(PDFLATEX) $(TARGETSTEM)

preamble.fmt: preamble.tex commands.tex
	$(PDFLATEX) -ini -jobname="preamble" "&pdflatex preamble.tex\dump"

again:
	make once

bg:
	make once > /dev/null &

twice:
	make once
	make once

figs:
	make -j 8 -f $(TARGETSTEM).makefile

ffigs:
	make -j 8 -B -f $(TARGETSTEM).makefile

bib:
	biber $(TARGETSTEM)

open:
	open -a skim $(TARGET)

clean:
	rm -rf *.{pdf,aux,log,out,bbl,wrt,toc,lof,lot,loe,figlist,makefile,listing,bcf,blg,capture,run.xml}
	rm -rf {frontmatter,backmatter}.aux preamble.fmt */main.aux externalized/*

all: once bib figs twice

new: clean once bib figs twice open


==> blocksize.tex <==
\begin{figure}\figurestyle
    \ref*{leg:cholbreakdown}

    \pgfplotsset{
        twocolplot,
        xlabel=block size $b$,
        table/search path={pred/figures/data/blockedbreakdown/},
        restrict x to domain=0:320,
    }

    \begin{subfigaxis}[
            fig caption=Accumulated kernel runtime,
            fig label=blocksize:breakdown,
            ylabel=runtime, y unit=\ms,
            stack plots=y,
            every axis plot/.append style={fill, fill opacity=.5},
        ]
        \addplot[blue] table[y=tdtrsm] {breakdown.dat} \closedcycle;
        \addplot[green] table[y=tdsyrk] {breakdown.dat} \closedcycle;
        \addplot[red] table[y=tdpotf2] {breakdown.dat} \closedcycle;
    \end{subfigaxis}\hfill
    \begin{subfigaxis}[
            fig caption=Average kernel performance,
            fig label=blocksize:perf,
            perfplot=52.8,
            legend to name=leg:cholbreakdown,
        ]
        \addplot[red] table[y=pdpotf2] {breakdown.dat};
        \addlegendentry{\dpotf[L]2}\label{plt:breakdown:dpotf2}
        \addplot[green] table[y=pdsyrk] {breakdown.dat};
        \addlegendentry{\dsyrk[LN]}\label{plt:breakdown:dsyrk}
        \addplot[blue] table[y=pdtrsm] {breakdown.dat};
        \addlegendentry{\dtrsm[RLTN]}\label{plt:breakdown:dtrsm}
    \end{subfigaxis}

    \mycaption{%
        Breakdown of the blocked Cholesky decomposition algorithm~3 in terms of
        kernel runtime and performance.
        \captiondetails{$n = 1000$, \haswell, 1~threads, \openblas, predictions}
    }
    \label{fig:pred:blocksize}
\end{figure}


==> intro/figures/algex.tex <==
\begin{figure}\figurestyle
    \pgfplotsset{
        every axis/.append style={
            twocolplot,
            xlabel={problem size},
            ylabel={performance},
            y unit=\si{\giga\flops\per\second},
        }
    }

    \begin{subfigure}\subfigwidth
        \raggedleft
        \tikzsetnextfilename{algex_sylv}
        \begin{tikzpicture}
            \begin{axis}[table/search path={model/figures/data/pred/sylv.penry.1}]
                \foreach \var/\i in {1/1, 2/2, 5/3, 6/4} {
                    \addplot table[y expr=2.5 * 8 * \thisrow{eff}]
                        {meas\var.med};
                    \label{plt:plot\i}
                }
            \end{axis}
        \end{tikzpicture}
        \caption{Sylvester equation solver}
        \label{fig:intro:algex:sylv}
    \end{subfigure}\hfill
    \begin{subfigure}\subfigwidth
        \raggedleft
        \tikzsetnextfilename{algex_tensor}
        \begin{tikzpicture}
            \begin{axis}[table/search path={tensor/figures/data/ijb_jcid10/meas}]
                \foreach \var in {169, ..., 176}
                    \addplot table {var\var.min};
            \end{axis}
        \end{tikzpicture}
        \caption{Tensor contractions}
        \label{fig:intro:algex:tensor}
    \end{subfigure}

    \mycaption{%
        Performance differences between alternative algorithms for the same
        operations with identical \flops counts.
    }
    \label{fig:intro:algex}
\end{figure}


==> intro/structure.tex <==
The remainder of this document is structured as follows:
\begin{itemize}
    \item \Cref{ch:meas} gives an overview of performance metrics and
        measurements.  It then introduces the \sampler: a flexible light-weight
        performance measurement tool for dense linear algebra routines.  This
        \sampler serves as a basis for the model generation, and
        micro-benchmarks presented in this work.  For interactive experiments,
        it is extended into the Experimental Linear Algebra Performance Studies
        framework (\elaps).

    \item \Cref{ch:model} covers the design and automatic generation of
        performance models.  These models are then used to rank and tune blocked
        algorithms for various operations.

    \item \cref{ch:cache} presents a study on the influence of caching on the
        runtime of compute kernels within dense linear algebra algorithms.

    \item \Cref{ch:tensor} is devoted to the prediction of \blas-based tensor
        contractions.  It describes the creation of cache-aware micro-benchmarks
        and presents

    \item \Cref{ch:conclusion} concludes the document, summarizes the results
        and gives an overview of potential future work.
\end{itemize}

The main content of this document is supplemented by two appendices:
\begin{itemize}
    \item \Cref{app:libs} gives an overview of the \blas and \lapack libraries,
        their kernels used in this work and several implementations.

    \item \Cref{app:hardware} lists the hardware setups used throughout this
        work and their properties.
\end{itemize}


==> pred/tables/bchol.tex <==
\begin{table}\tablestyle
    \begin{tabular}{clcccc}
        \toprule
        &&$n = 1000$ &$n = 2000$ &$n = 3000$ &$n = 4000$ \\
        &&(\ref*{plt:n1000}) &(\ref*{plt:n2000}) &(\ref*{plt:n3000}) &(\ref*{plt:n4000}) \\
        \midrule
        \multirow3*{1 thread}
        \input{pred/figures/data/bchol/tablest}
        \midrule
        \multirow3*{12 threads}
        \input{pred/figures/data/bchol/tablemt}
        \bottomrule
    \end{tabular}
    \mycaption{
        Empirical and predicted optimal block sizes and yields for of the
        Cholesky decomposition blocked algorithm~3.
        \captiondetails{\haswell, \openblas}
    }
    \label{tbl:pred:b:chol}
\end{table}


==> pred/tables/blu.tex <==
\begin{table}\tablestyle
    \begin{tabular}{clcccc}
        \toprule
        &&$n = 1000$ &$n = 2000$ &$n = 3000$ &$n = 4000$ \\
        &&(\ref*{plt:n1000}) &(\ref*{plt:n2000}) &(\ref*{plt:n3000}) &(\ref*{plt:n4000}) \\
        \midrule
        \multirow4*{1 thread}
        \input{pred/figures/data/blu/tablest}
        \midrule
        \multirow4*{12 threads}
        \input{pred/figures/data/blu/tablemt}
        \bottomrule
    \end{tabular}
    \mycaption{
        Empirical and predicted optimal block sizes and yields for \lapack's
        blocked LU~decomposition \dgetrf.
        \captiondetails{\haswell, \openblas}
    }
    \label{tbl:pred:b:lu}
\end{table}


==> pred/tables/bqr.tex <==
\begin{table}\tablestyle
    \begin{tabular}{clcccc}
        \toprule
        &&$n = 1000$ &$n = 2000$ &$n = 3000$ &$n = 4000$ \\
        &&(\ref*{plt:n1000}) &(\ref*{plt:n2000}) &(\ref*{plt:n3000}) &(\ref*{plt:n4000}) \\
        \midrule
        \multirow4*{1 thread}
        \input{pred/figures/data/bqr/tablest}
        \midrule
        \multirow4*{12 threads}
        \input{pred/figures/data/bqr/tablemt}
        \bottomrule
    \end{tabular}
    \mycaption{
        Empirical and predicted optimal block sizes and yields for \lapack's
        blocked QR~decomposition \dgeqrf.
        \captiondetails{\haswell, \openblas}
    }
    \label{tbl:pred:b:qr}
\end{table}


==> pred/tables/btrinv.tex <==
\begin{table}\tablestyle
    \begin{tabular}{clcccc}
        \toprule
        &&$n = 1000$ &$n = 2000$ &$n = 3000$ &$n = 4000$ \\
        &&(\ref*{plt:n1000}) &(\ref*{plt:n2000}) &(\ref*{plt:n3000}) &(\ref*{plt:n4000}) \\
        \midrule
        \multirow3*{1 thread}
        \input{pred/figures/data/btrinv/tablest}
        \midrule
        \multirow3*{12 threads}
        \input{pred/figures/data/btrinv/tablemt}
        \bottomrule
    \end{tabular}
    \mycaption{
        Empirical and predicted optimal block sizes and yields for the
        inversion of a lower-triangular matrix blocked algorithm 3.
        \captiondetails{\haswell, \openblas}
    }
    \label{tbl:pred:b:trinv}
\end{table}

